Measurement of exclusive $\gamma\gamma\rightarrow W^+W^-$ production and search for exclusive Higgs boson production in $pp$ collisions at $\sqrt{s} = 8$ TeV using the ATLAS detector

Searches for exclusively produced $W$ boson pairs in the process $pp(\gamma\gamma) \rightarrow pW^+W^-p$ and exclusively produced Higgs boson in the process $pp(gg) \rightarrow pHp$ have been performed using $e^{\pm}\mu^{\mp}$ final states. These measurements use 20.2 fb$^{-1}$ of $pp$ collisions collected by the ATLAS experiment at a center-of-mass energy $\sqrt{s}=8$ TeV at the LHC. Exclusive production of $W^+W^-$ consistent with the Standard Model prediction is found with 3.0$\sigma$ significance. The exclusive $W^+W^-$ production cross-section is determined to be $\sigma (\gamma\gamma\rightarrow W^{+}W^{-}\rightarrow e^{\pm}\mu^{\mp} X) = 6.9 \pm 2.2 (\mathrm{stat.}) \pm 1.4 (\mathrm{sys.})$ fb, in agreement with the Standard Model prediction. Limits on anomalous quartic gauge couplings are set at 95\% confidence-level as $-1.7 \times 10^{-6} < a_0^W/\Lambda^2 < 1.7 \times 10^{-6}$ GeV$^{-2}$and $-6.4 \times 10^{-6} < a_C^W/\Lambda^2 < 6.3 \times 10^{-6}$ GeV$^{-2}$. A 95\% confidence-level upper limit on the total production cross-section for exclusive Higgs boson is set to 1.2 pb.

==> Acknowledgements.tex <==
% Acknowledgements for papers with collision data
% Version 2-Aug-2016

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC, Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP, Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC, China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic; DNRF and DNSRC, Denmark; IN2P3-CNRS, CEA-DSM/IRFU, France; GNSF, Georgia; BMBF, HGF, and MPG, Germany; GSRT, Greece; RGC, Hong Kong SAR, China; ISF, I-CORE and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; FOM and NWO, Netherlands; RCN, Norway; MNiSW and NCN, Poland; FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MESTD, Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa; MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SERI, SNSF and Cantons of Bern and Geneva, Switzerland; MOST, Taiwan; TAEK, Turkey; STFC, United Kingdom; DOE and NSF, United States of America. In addition, individual groups and members have received support from BCKDF, the Canada Council, CANARIE, CRC, Compute Canada, FQRNT, and the Ontario Innovation Trust, Canada; EPLANET, ERC, FP7, Horizon 2020 and Marie Sk{\l}odowska-Curie Actions, European Union; Investissements d'Avenir Labex and Idex, ANR, R{\'e}gion Auvergne and Fondation Partager le Savoir, France; DFG and AvH Foundation, Germany; Herakleitos, Thales and Aristeia programmes co-financed by EU-ESF and the Greek NSRF; BSF, GIF and Minerva, Israel; BRF, Norway; Generalitat de Catalunya, Generalitat Valenciana, Spain; the Royal Society and Leverhulme Trust, United Kingdom.

The crucial computing support from all WLCG partners is acknowledged gratefully, in particular from CERN, the ATLAS Tier-1 facilities at TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France), KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain), ASGC (Taiwan), RAL (UK) and BNL (USA), the Tier-2 facilities worldwide and large non-WLCG resource providers. Major contributors of computing resources are listed in Ref.~\cite{ATL-GEN-PUB-2016-002}.
%----------------------------------------------


